Interior over-penalized enriched Galerkin methods for second order elliptic equations

In this paper we propose a variant of enriched Galerkin methods for second order elliptic equations with over-penalization of interior jump terms. The bilinear form with interior over-penalization gives a non-standard norm which is different from the discrete energy norm in the classical discontinuous Galerkin methods. Nonetheless we prove that optimal a priori error estimates with the standard discrete energy norm can be obtained by combining a priori and a posteriori error analysis techniques. We also show that the interior over-penalization is advantageous for constructing preconditioners robust to mesh refinement by analyzing spectral equivalence of bilinear forms. Numerical results are included to illustrate the convergence and preconditioning results.

==> code/results-08-11-2023/iop-eg-precond-result-fd-gmres-01.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = iop-eg
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$15~(0.3)$ &$15~(0.05)$ &$15~(0.13)$ &$14~(0.22)$ &$14~(0.89)$ \\ 
			\multirow{4}{*}{$1$} & $ 2$ &$17~(0.04)$ &$17~(0.05)$ &$16~(0.07)$ &$16~(0.24)$ &$15~(1.04)$ \\ 
			&$4$ &$19~(0.04)$ &$18~(0.05)$ &$18~(0.07)$ &$17~(0.24)$ &$17~(1.13)$ \\ 
			&$8$ &$25~(0.05)$ &$27~(0.06)$ &$25~(0.1)$ &$24~(0.27)$ &$22~(1.04)$ \\ 
			\cline{2-7} 
			&$1$ &$23~(0.23)$ &$22~(0.06)$ &$21~(0.17)$ &$19~(0.64)$ &$17~(2.77)$ \\ 
			\multirow{4}{*}{$2$} & $ 2$ &$53~(0.07)$ &$48~(0.08)$ &$46~(0.26)$ &$39~(0.93)$ &$27~(3.4)$ \\ 
			&$4$ &$107~(0.07)$ &$103~(0.08)$ &$79~(0.33)$ &$69~(1.13)$ &$47~(3.94)$ \\ 
			&$8$ &$208~(0.12)$ &$774~(0.43)$ &$869~(1.86)$ &$76~(1.13)$ &$60~(4.64)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 1$} 
		\label{table:iop-eg} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iop-eg-precond-result-fd-gmres-02.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = cubic
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$12~(0.3)$ &$11~(0.05)$ &$10~(0.12)$ &$9~(0.22)$ &$9~(0.82)$ \\ 
			\multirow{4}{*}{$1$} & $ 2$ &$13~(0.04)$ &$12~(0.05)$ &$11~(0.07)$ &$11~(0.23)$ &$10~(0.84)$ \\ 
			&$4$ &$15~(0.04)$ &$15~(0.05)$ &$14~(0.07)$ &$13~(0.22)$ &$12~(0.88)$ \\ 
			&$8$ &$20~(0.04)$ &$22~(0.05)$ &$22~(0.07)$ &$20~(0.25)$ &$19~(1.05)$ \\ 
			\cline{2-7} 
			&$1$ &$21~(0.23)$ &$18~(0.06)$ &$17~(0.16)$ &$15~(0.59)$ &$13~(2.68)$ \\ 
			\multirow{4}{*}{$2$} & $ 2$ &$41~(0.06)$ &$47~(0.08)$ &$45~(0.22)$ &$36~(0.77)$ &$22~(2.94)$ \\ 
			&$4$ &$68~(0.06)$ &$80~(0.08)$ &$66~(0.25)$ &$56~(0.94)$ &$44~(4.1)$ \\ 
			&$8$ &$101~(0.06)$ &$119~(0.19)$ &$90~(0.3)$ &$63~(1.15)$ &$50~(4.35)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 2$} 
		\label{table:cubic} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iop-eg-precond-result-fd-gmres-03.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = quartic
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$10~(0.32)$ &$10~(0.05)$ &$9~(0.12)$ &$9~(0.3)$ &$8~(0.97)$ \\ 
			\multirow{4}{*}{$1$} & $ 2$ &$12~(0.06)$ &$11~(0.06)$ &$11~(0.09)$ &$10~(0.25)$ &$10~(0.93)$ \\ 
			&$4$ &$14~(0.04)$ &$14~(0.05)$ &$13~(0.07)$ &$13~(0.23)$ &$12~(1.07)$ \\ 
			&$8$ &$18~(0.05)$ &$21~(0.09)$ &$21~(0.08)$ &$20~(0.3)$ &$18~(1.06)$ \\ 
			\cline{2-7} 
			&$1$ &$20~(0.22)$ &$18~(0.05)$ &$16~(0.16)$ &$15~(0.57)$ &$13~(2.85)$ \\ 
			\multirow{4}{*}{$2$} & $ 2$ &$38~(0.05)$ &$46~(0.07)$ &$44~(0.19)$ &$35~(0.72)$ &$22~(3.06)$ \\ 
			&$4$ &$57~(0.05)$ &$75~(0.07)$ &$65~(0.24)$ &$55~(0.97)$ &$44~(3.92)$ \\ 
			&$8$ &$71~(0.06)$ &$110~(0.2)$ &$90~(0.28)$ &$60~(1.01)$ &$49~(4.0)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 3$} 
		\label{table:quartic} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iop-eg-precond-result-fd-gmres-04.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = large
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$14~(0.28)$ &$16~(0.04)$ &$18~(0.12)$ &$21~(0.26)$ &$25~(1.06)$ \\ 
			\multirow{4}{*}{$1$} & $ 2$ &$15~(0.04)$ &$17~(0.05)$ &$20~(0.07)$ &$24~(0.25)$ &$29~(1.11)$ \\ 
			&$4$ &$17~(0.04)$ &$20~(0.04)$ &$22~(0.07)$ &$26~(0.29)$ &$35~(1.22)$ \\ 
			&$8$ &$23~(0.04)$ &$27~(0.05)$ &$30~(0.08)$ &$37~(0.3)$ &$42~(1.5)$ \\ 
			\cline{2-7} 
			&$1$ &$22~(0.22)$ &$22~(0.05)$ &$24~(0.16)$ &$25~(0.64)$ &$28~(3.01)$ \\ 
			\multirow{4}{*}{$2$} & $ 2$ &$51~(0.05)$ &$48~(0.06)$ &$47~(0.2)$ &$46~(0.94)$ &$42~(3.66)$ \\ 
			&$4$ &$78~(0.05)$ &$99~(0.08)$ &$94~(0.29)$ &$90~(1.24)$ &$171~(8.48)$ \\ 
			&$8$ &$150~(0.06)$ &$1181~(0.56)$ &$672~(1.3)$ &$236~(2.43)$ &$260~(11.68)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 0$} 
		\label{table:large} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iop-eg-precond-result-fd-gmres-05.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = onehalf
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$19~(0.29)$ &$22~(0.05)$ &$22~(0.12)$ &$24~(0.25)$ &$25~(1.05)$ \\ 
			\multirow{4}{*}{$1$} & $ 2$ &$22~(0.04)$ &$24~(0.05)$ &$26~(0.07)$ &$28~(0.27)$ &$30~(1.12)$ \\ 
			&$4$ &$24~(0.04)$ &$26~(0.05)$ &$28~(0.08)$ &$30~(0.27)$ &$36~(1.22)$ \\ 
			&$8$ &$44~(0.04)$ &$43~(0.07)$ &$43~(0.09)$ &$42~(0.33)$ &$46~(1.61)$ \\ 
			\cline{2-7} 
			&$1$ &$26~(0.25)$ &$27~(0.07)$ &$28~(0.18)$ &$28~(0.72)$ &$28~(3.24)$ \\ 
			\multirow{4}{*}{$2$} & $ 2$ &$65~(0.05)$ &$53~(0.08)$ &$52~(0.22)$ &$53~(0.93)$ &$43~(3.84)$ \\ 
			&$4$ &$178~(0.07)$ &$149~(0.09)$ &$150~(0.38)$ &$161~(1.88)$ &$177~(8.7)$ \\ 
			&$8$ &$1016~(0.17)$ &$643~(0.36)$ &$884~(1.81)$ &$377~(3.79)$ &$257~(12.54)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 0.5$} 
		\label{table:onehalf} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iop-eg-precond-result-fd-gmres-06.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = one95
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$16~(0.28)$ &$16~(0.05)$ &$15~(0.12)$ &$15~(0.22)$ &$14~(0.9)$ \\ 
			\multirow{4}{*}{$1$} & $ 2$ &$17~(0.04)$ &$17~(0.04)$ &$17~(0.07)$ &$16~(0.23)$ &$16~(0.91)$ \\ 
			&$4$ &$19~(0.04)$ &$20~(0.04)$ &$19~(0.07)$ &$18~(0.23)$ &$17~(0.93)$ \\ 
			&$8$ &$26~(0.05)$ &$27~(0.05)$ &$26~(0.08)$ &$24~(0.32)$ &$22~(1.06)$ \\ 
			\cline{2-7} 
			&$1$ &$23~(0.24)$ &$22~(0.05)$ &$21~(0.16)$ &$20~(0.6)$ &$18~(2.66)$ \\ 
			\multirow{4}{*}{$2$} & $ 2$ &$54~(0.05)$ &$48~(0.06)$ &$46~(0.21)$ &$40~(0.77)$ &$27~(2.98)$ \\ 
			&$4$ &$113~(0.05)$ &$99~(0.08)$ &$82~(0.26)$ &$69~(1.02)$ &$48~(3.77)$ \\ 
			&$8$ &$244~(0.07)$ &$1009~(0.47)$ &$7012~(14.43)$ &$77~(1.11)$ &$65~(4.68)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 0.95$} 
		\label{table:one95} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_iop-eg-precond-exp-fd-08-07-2023.py-cubic.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = cubic
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$15~(0.29)$ &$15~(0.06)$ &$14~(0.08)$ &$14~(0.24)$ &$13~(0.96)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$15~(0.05)$ &$15~(0.05)$ &$14~(0.07)$ &$14~(0.24)$ &$14~(0.91)$ \\ 
			&$4$ &$16~(0.05)$ &$15~(0.05)$ &$15~(0.07)$ &$14~(0.22)$ &$14~(1.16)$ \\ 
			&$8$ &$16~(0.06)$ &$15~(0.06)$ &$15~(0.07)$ &$15~(0.28)$ &$14~(1.0)$ \\ 
			&$10$ &$16~(0.05)$ &$16~(0.09)$ &$15~(0.07)$ &$15~(0.24)$ &$14~(1.03)$ \\ 
			\cline{2-7} 
			&$1$ &$28~(0.26)$ &$29~(0.06)$ &$29~(0.19)$ &$27~(0.82)$ &$25~(3.29)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$29~(0.05)$ &$30~(0.06)$ &$29~(0.18)$ &$29~(0.78)$ &$28~(3.05)$ \\ 
			&$4$ &$31~(0.06)$ &$31~(0.06)$ &$30~(0.17)$ &$29~(0.76)$ &$29~(3.02)$ \\ 
			&$8$ &$31~(0.05)$ &$31~(0.06)$ &$31~(0.17)$ &$30~(0.78)$ &$29~(3.34)$ \\ 
			&$10$ &$32~(0.05)$ &$31~(0.12)$ &$31~(0.25)$ &$30~(1.05)$ &$29~(3.37)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 2$ : New cubic
		} 
		\label{table:cubic} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_iop-eg-precond-exp-fd-08-07-2023.py-eg.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = eg
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$27~(0.29)$ &$36~(0.05)$ &$48~(0.1)$ &$64~(0.4)$ &$86~(2.24)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$29~(0.05)$ &$37~(0.06)$ &$50~(0.11)$ &$67~(0.4)$ &$91~(2.22)$ \\ 
			&$4$ &$29~(0.05)$ &$40~(0.05)$ &$54~(0.1)$ &$73~(0.44)$ &$99~(2.24)$ \\ 
			&$8$ &$30~(0.05)$ &$43~(0.05)$ &$59~(0.13)$ &$81~(0.47)$ &$110~(2.37)$ \\ 
			&$10$ &$30~(0.05)$ &$43~(0.06)$ &$59~(0.12)$ &$83~(0.51)$ &$115~(2.72)$ \\ 
			\cline{2-7} 
			&$1$ &$38~(0.24)$ &$45~(0.08)$ &$56~(0.21)$ &$73~(1.23)$ &$95~(5.38)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$40~(0.07)$ &$47~(0.09)$ &$59~(0.29)$ &$76~(1.15)$ &$101~(5.55)$ \\ 
			&$4$ &$42~(0.05)$ &$51~(0.07)$ &$63~(0.23)$ &$83~(1.15)$ &$110~(6.16)$ \\ 
			&$8$ &$45~(0.05)$ &$55~(0.07)$ &$70~(0.29)$ &$93~(1.33)$ &$124~(6.84)$ \\ 
			&$10$ &$46~(0.05)$ &$57~(0.1)$ &$72~(0.27)$ &$97~(1.29)$ &$129~(6.74)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 0$ : New EG} 
		\label{table:eg} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_iop-eg-precond-exp-fd-08-07-2023.py-iop-eg.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = iop-eg
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$17~(0.44)$ &$18~(0.07)$ &$19~(0.09)$ &$19~(0.33)$ &$18~(1.03)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$18~(0.06)$ &$19~(0.05)$ &$19~(0.08)$ &$19~(0.25)$ &$19~(1.04)$ \\ 
			&$4$ &$19~(0.05)$ &$20~(0.08)$ &$20~(0.12)$ &$19~(0.3)$ &$19~(1.07)$ \\ 
			&$8$ &$20~(0.05)$ &$21~(0.05)$ &$21~(0.09)$ &$21~(0.28)$ &$20~(1.06)$ \\ 
			&$10$ &$20~(0.05)$ &$21~(0.05)$ &$21~(0.07)$ &$21~(0.24)$ &$21~(1.03)$ \\ 
			\cline{2-7} 
			&$1$ &$31~(0.24)$ &$32~(0.06)$ &$31~(0.17)$ &$30~(0.8)$ &$28~(3.08)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$32~(0.05)$ &$33~(0.06)$ &$33~(0.19)$ &$32~(0.79)$ &$30~(3.24)$ \\ 
			&$4$ &$33~(0.06)$ &$34~(0.08)$ &$34~(0.18)$ &$32~(0.75)$ &$32~(3.27)$ \\ 
			&$8$ &$34~(0.05)$ &$35~(0.06)$ &$35~(0.2)$ &$34~(0.83)$ &$33~(3.48)$ \\ 
			&$10$ &$35~(0.05)$ &$36~(0.11)$ &$35~(0.24)$ &$34~(0.84)$ &$33~(3.44)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 1$ : New iop-eg
		} 
		\label{table:iop-eg} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_iop-eg-precond-exp-fd-08-07-2023.py-large.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = large
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$15~(0.3)$ &$17~(0.05)$ &$19~(0.08)$ &$22~(0.25)$ &$25~(1.06)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$16~(0.05)$ &$17~(0.05)$ &$20~(0.07)$ &$23~(0.25)$ &$26~(1.06)$ \\ 
			&$4$ &$16~(0.09)$ &$18~(0.08)$ &$20~(0.09)$ &$23~(0.29)$ &$28~(1.17)$ \\ 
			&$8$ &$17~(0.05)$ &$19~(0.06)$ &$21~(0.08)$ &$25~(0.33)$ &$31~(1.19)$ \\ 
			&$10$ &$17~(0.05)$ &$19~(0.06)$ &$22~(0.08)$ &$26~(0.29)$ &$32~(1.32)$ \\ 
			\cline{2-7} 
			&$1$ &$29~(0.26)$ &$31~(0.06)$ &$31~(0.18)$ &$32~(0.88)$ &$35~(3.32)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$30~(0.05)$ &$32~(0.07)$ &$33~(0.18)$ &$34~(0.83)$ &$37~(3.45)$ \\ 
			&$4$ &$31~(0.05)$ &$33~(0.06)$ &$34~(0.18)$ &$35~(0.73)$ &$38~(3.46)$ \\ 
			&$8$ &$32~(0.06)$ &$34~(0.07)$ &$35~(0.21)$ &$37~(0.83)$ &$41~(3.6)$ \\ 
			&$10$ &$32~(0.05)$ &$34~(0.08)$ &$35~(0.21)$ &$37~(0.85)$ &$41~(4.23)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 0$ : New large
		} 
		\label{table:large} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_iop-eg-precond-exp-fd-08-07-2023.py-one6.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = one6
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$20~(52.11)$ &$23~(0.1)$ &$24~(0.21)$ &$26~(0.72)$ &$28~(2.21)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$21~(0.15)$ &$23~(0.2)$ &$25~(0.14)$ &$27~(0.54)$ &$29~(2.11)$ \\ 
			&$4$ &$22~(0.21)$ &$25~(0.13)$ &$27~(0.25)$ &$29~(0.56)$ &$31~(2.15)$ \\ 
			&$8$ &$23~(0.1)$ &$27~(0.11)$ &$29~(0.16)$ &$32~(0.62)$ &$34~(2.87)$ \\ 
			&$10$ &$23~(0.1)$ &$27~(0.12)$ &$30~(0.16)$ &$33~(0.73)$ &$35~(2.37)$ \\ 
			\cline{2-7} 
			&$1$ &$33~(37.39)$ &$33~(0.17)$ &$34~(0.38)$ &$36~(1.64)$ &$37~(6.08)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$34~(0.1)$ &$36~(0.27)$ &$37~(0.43)$ &$38~(1.56)$ &$39~(6.21)$ \\ 
			&$4$ &$35~(0.09)$ &$38~(0.12)$ &$38~(0.35)$ &$39~(1.55)$ &$40~(6.8)$ \\ 
			&$8$ &$37~(0.15)$ &$39~(0.15)$ &$41~(0.38)$ &$42~(1.7)$ &$44~(7.03)$ \\ 
			&$10$ &$38~(0.15)$ &$40~(0.15)$ &$42~(0.45)$ &$44~(1.55)$ &$45~(6.63)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 0.6000000000000001$} 
		\label{table:one6} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_iop-eg-precond-exp-fd-08-07-2023.py-one7.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = one7
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$19~(17.59)$ &$21~(0.13)$ &$23~(0.15)$ &$23~(0.53)$ &$24~(2.53)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$20~(0.1)$ &$22~(0.11)$ &$23~(0.2)$ &$25~(0.52)$ &$25~(2.08)$ \\ 
			&$4$ &$21~(0.12)$ &$23~(0.18)$ &$25~(0.15)$ &$26~(0.66)$ &$26~(2.0)$ \\ 
			&$8$ &$22~(0.1)$ &$25~(0.1)$ &$27~(0.16)$ &$28~(0.57)$ &$29~(2.05)$ \\ 
			&$10$ &$22~(0.1)$ &$26~(0.24)$ &$27~(0.15)$ &$29~(0.55)$ &$30~(2.11)$ \\ 
			\cline{2-7} 
			&$1$ &$32~(6.91)$ &$33~(0.12)$ &$33~(0.39)$ &$33~(1.69)$ &$33~(7.38)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$34~(0.1)$ &$35~(0.12)$ &$35~(0.35)$ &$36~(1.78)$ &$36~(6.23)$ \\ 
			&$4$ &$35~(0.1)$ &$37~(0.16)$ &$37~(0.4)$ &$37~(1.95)$ &$37~(8.25)$ \\ 
			&$8$ &$36~(0.19)$ &$38~(0.15)$ &$39~(0.4)$ &$39~(1.88)$ &$40~(6.92)$ \\ 
			&$10$ &$37~(0.09)$ &$38~(0.12)$ &$39~(0.4)$ &$40~(1.74)$ &$41~(6.16)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 0.7$} 
		\label{table:one7} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_iop-eg-precond-exp-fd-08-07-2023.py-one8.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = one8
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$18~(16.29)$ &$20~(0.09)$ &$21~(0.23)$ &$21~(0.58)$ &$22~(2.02)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$19~(0.1)$ &$21~(0.1)$ &$22~(0.15)$ &$22~(0.56)$ &$23~(2.08)$ \\ 
			&$4$ &$20~(0.14)$ &$22~(0.09)$ &$23~(0.16)$ &$23~(0.54)$ &$23~(2.11)$ \\ 
			&$8$ &$21~(0.09)$ &$24~(0.12)$ &$24~(0.15)$ &$25~(0.75)$ &$26~(2.29)$ \\ 
			&$10$ &$22~(0.12)$ &$24~(0.26)$ &$25~(0.15)$ &$26~(0.56)$ &$26~(2.13)$ \\ 
			\cline{2-7} 
			&$1$ &$32~(6.74)$ &$33~(0.13)$ &$32~(0.35)$ &$31~(1.26)$ &$31~(5.53)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$33~(0.11)$ &$35~(0.18)$ &$34~(0.33)$ &$34~(1.56)$ &$34~(6.05)$ \\ 
			&$4$ &$35~(0.1)$ &$36~(0.15)$ &$36~(0.39)$ &$35~(1.32)$ &$35~(6.46)$ \\ 
			&$8$ &$35~(0.09)$ &$37~(0.12)$ &$37~(0.34)$ &$37~(1.47)$ &$36~(6.45)$ \\ 
			&$10$ &$36~(0.13)$ &$37~(0.17)$ &$37~(0.54)$ &$37~(2.08)$ &$37~(7.18)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 0.8$} 
		\label{table:one8} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_iop-eg-precond-exp-fd-08-07-2023.py-one9.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = one9
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$18~(6.37)$ &$19~(0.05)$ &$20~(0.08)$ &$20~(0.25)$ &$20~(0.97)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$19~(0.05)$ &$20~(0.05)$ &$20~(0.08)$ &$20~(0.24)$ &$20~(1.03)$ \\ 
			&$4$ &$20~(0.05)$ &$21~(0.05)$ &$21~(0.1)$ &$21~(0.29)$ &$21~(0.99)$ \\ 
			&$8$ &$20~(0.05)$ &$22~(0.05)$ &$22~(0.07)$ &$23~(0.26)$ &$23~(1.13)$ \\ 
			&$10$ &$21~(0.05)$ &$23~(0.06)$ &$23~(0.09)$ &$23~(0.29)$ &$23~(1.05)$ \\ 
			\cline{2-7} 
			&$1$ &$31~(2.86)$ &$33~(0.07)$ &$31~(0.19)$ &$30~(0.71)$ &$30~(3.05)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$33~(0.05)$ &$34~(0.06)$ &$33~(0.18)$ &$33~(0.75)$ &$32~(3.32)$ \\ 
			&$4$ &$34~(0.05)$ &$35~(0.06)$ &$35~(0.21)$ &$34~(0.81)$ &$33~(3.28)$ \\ 
			&$8$ &$35~(0.05)$ &$36~(0.06)$ &$36~(0.18)$ &$35~(0.84)$ &$35~(3.33)$ \\ 
			&$10$ &$35~(0.07)$ &$36~(0.08)$ &$36~(0.25)$ &$35~(0.75)$ &$35~(3.32)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 0.9$} 
		\label{table:one9} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_iop-eg-precond-exp-fd-08-07-2023.py-one95.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = one95
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$17~(0.28)$ &$19~(0.06)$ &$19~(0.12)$ &$19~(0.24)$ &$19~(0.97)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$19~(0.05)$ &$20~(0.06)$ &$20~(0.07)$ &$20~(0.24)$ &$19~(1.0)$ \\ 
			&$4$ &$19~(0.05)$ &$20~(0.05)$ &$20~(0.08)$ &$20~(0.24)$ &$20~(0.98)$ \\ 
			&$8$ &$20~(0.05)$ &$22~(0.05)$ &$22~(0.09)$ &$22~(0.26)$ &$22~(1.02)$ \\ 
			&$10$ &$21~(0.05)$ &$22~(0.06)$ &$22~(0.08)$ &$22~(0.26)$ &$22~(1.04)$ \\ 
			\cline{2-7} 
			&$1$ &$31~(2.87)$ &$32~(0.06)$ &$31~(0.22)$ &$30~(0.7)$ &$29~(3.1)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$33~(0.05)$ &$33~(0.06)$ &$33~(0.22)$ &$32~(0.75)$ &$31~(3.18)$ \\ 
			&$4$ &$34~(0.05)$ &$34~(0.06)$ &$34~(0.21)$ &$33~(0.84)$ &$33~(3.26)$ \\ 
			&$8$ &$34~(0.05)$ &$36~(0.06)$ &$35~(0.18)$ &$34~(0.77)$ &$34~(3.33)$ \\ 
			&$10$ &$35~(0.06)$ &$36~(0.06)$ &$35~(0.22)$ &$35~(0.76)$ &$34~(3.28)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 0.95$
		} 
		\label{table:one95} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_iop-eg-precond-exp-fd-08-07-2023.py-onehalf.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = onehalf
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$21~(0.3)$ &$23~(0.06)$ &$26~(0.09)$ &$29~(0.31)$ &$32~(1.22)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$22~(0.05)$ &$25~(0.05)$ &$27~(0.09)$ &$31~(0.3)$ &$34~(1.33)$ \\ 
			&$4$ &$23~(0.05)$ &$27~(0.06)$ &$30~(0.09)$ &$33~(0.31)$ &$37~(1.36)$ \\ 
			&$8$ &$24~(0.05)$ &$29~(0.05)$ &$32~(0.11)$ &$36~(0.37)$ &$41~(1.44)$ \\ 
			&$10$ &$24~(0.06)$ &$29~(0.06)$ &$34~(0.1)$ &$38~(0.34)$ &$42~(1.49)$ \\ 
			\cline{2-7} 
			&$1$ &$34~(0.25)$ &$35~(0.07)$ &$37~(0.26)$ &$39~(0.91)$ &$41~(3.46)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$35~(0.06)$ &$37~(0.07)$ &$39~(0.19)$ &$40~(0.83)$ &$42~(3.57)$ \\ 
			&$4$ &$36~(0.05)$ &$39~(0.06)$ &$40~(0.19)$ &$42~(0.8)$ &$45~(3.95)$ \\ 
			&$8$ &$38~(0.06)$ &$41~(0.07)$ &$44~(0.19)$ &$46~(0.81)$ &$48~(3.76)$ \\ 
			&$10$ &$39~(0.05)$ &$42~(0.09)$ &$45~(0.23)$ &$47~(0.94)$ &$51~(4.12)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 0.5$} 
		\label{table:onehalf} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_iop-eg-precond-exp-fd-08-07-2023.py-quartic.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = quartic
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$14~(0.3)$ &$14~(0.06)$ &$14~(0.08)$ &$13~(0.24)$ &$13~(0.94)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$14~(0.06)$ &$14~(0.06)$ &$14~(0.09)$ &$14~(0.23)$ &$13~(1.06)$ \\ 
			&$4$ &$14~(0.05)$ &$14~(0.05)$ &$14~(0.07)$ &$14~(0.25)$ &$14~(0.93)$ \\ 
			&$8$ &$14~(0.05)$ &$15~(0.05)$ &$14~(0.08)$ &$14~(0.27)$ &$58~(1.57)$ \\ 
			&$10$ &$15~(0.05)$ &$15~(0.05)$ &$14~(0.07)$ &$14~(0.22)$ &$14~(0.86)$ \\ 
			\cline{2-7} 
			&$1$ &$28~(0.23)$ &$29~(0.07)$ &$28~(0.17)$ &$26~(0.8)$ &$26~(3.09)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$29~(0.05)$ &$29~(0.06)$ &$29~(0.18)$ &$28~(0.75)$ &$28~(3.16)$ \\ 
			&$4$ &$30~(0.05)$ &$30~(0.07)$ &$30~(0.18)$ &$29~(0.7)$ &$28~(3.17)$ \\ 
			&$8$ &$30~(0.07)$ &$31~(0.08)$ &$30~(0.19)$ &$30~(0.86)$ &$58~(4.41)$ \\ 
			&$10$ &$30~(0.08)$ &$30~(0.09)$ &$30~(0.22)$ &$30~(0.83)$ &$29~(3.41)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 3$} 
		\label{table:quartic} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_tmp-eg-precond-code.py-iop-eg.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = iop-eg
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$17~(0.31)$ &$18~(0.05)$ &$19~(0.08)$ &$19~(0.24)$ &$18~(0.93)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$18~(0.05)$ &$19~(0.06)$ &$19~(0.08)$ &$19~(0.26)$ &$19~(0.98)$ \\ 
			&$4$ &$19~(0.05)$ &$20~(0.05)$ &$20~(0.09)$ &$19~(0.24)$ &$19~(0.99)$ \\ 
			&$8$ &$20~(0.05)$ &$21~(0.05)$ &$21~(0.08)$ &$21~(0.3)$ &$20~(0.97)$ \\ 
			&$10$ &$20~(0.05)$ &$21~(0.05)$ &$21~(0.09)$ &$21~(0.3)$ &$21~(0.99)$ \\ 
			\cline{2-7} 
			&$1$ &$31~(0.25)$ &$32~(0.07)$ &$31~(0.18)$ &$30~(0.78)$ &$28~(3.18)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$32~(0.05)$ &$33~(0.06)$ &$33~(0.18)$ &$32~(0.77)$ &$30~(3.08)$ \\ 
			&$4$ &$33~(0.05)$ &$34~(0.06)$ &$34~(0.18)$ &$32~(0.74)$ &$32~(3.28)$ \\ 
			&$8$ &$34~(0.05)$ &$35~(0.06)$ &$35~(0.18)$ &$34~(0.75)$ &$33~(3.63)$ \\ 
			&$10$ &$35~(0.05)$ &$36~(0.09)$ &$35~(0.19)$ &$34~(1.04)$ &$33~(3.49)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 1$} 
		\label{table:iop-eg} 
	\end{center} 
\end{table} 


==> code/results-08-11-2023/iteration_result_tmp-eg-precond-code.py.tex <==
% EG precond test 
%% tensor [[k00 k01], [k01, k11]] = [[1.0,0],[0,1.0]]
%% method = iop-eg
\begin{table}[h]
	\begin{center}
		\begin{tabular}{c|c||c c c c c} 
			\multicolumn{2}{c||}{ } & \multicolumn{5}{c}{$N$} \\ 
			$k$ &$\ \kappa_0$ &$8$ &$16$ &$32$ &$64$ &$128$ \\ 
			\hline 
			&$1$ &$17~(13.82)$ &$18~(0.05)$ &$19~(0.08)$ &$19~(0.25)$ &$18~(0.98)$ \\ 
			\multirow{5}{*}{$1$} & $ 2$ &$18~(0.05)$ &$19~(0.05)$ &$19~(0.15)$ &$19~(0.26)$ &$19~(0.95)$ \\ 
			&$4$ &$19~(0.05)$ &$20~(0.05)$ &$20~(0.07)$ &$19~(0.24)$ &$19~(0.95)$ \\ 
			&$8$ &$20~(0.06)$ &$21~(0.06)$ &$21~(0.08)$ &$21~(0.24)$ &$20~(1.06)$ \\ 
			&$10$ &$20~(0.05)$ &$21~(0.05)$ &$21~(0.08)$ &$21~(0.24)$ &$21~(1.09)$ \\ 
			\cline{2-7} 
			&$1$ &$31~(9.44)$ &$32~(0.07)$ &$31~(0.18)$ &$30~(0.7)$ &$28~(2.98)$ \\ 
			\multirow{5}{*}{$2$} & $ 2$ &$32~(0.07)$ &$33~(0.08)$ &$33~(0.23)$ &$32~(0.76)$ &$30~(3.33)$ \\ 
			&$4$ &$33~(0.06)$ &$34~(0.07)$ &$34~(0.21)$ &$32~(0.87)$ &$32~(3.77)$ \\ 
			&$8$ &$34~(0.05)$ &$35~(0.06)$ &$35~(0.2)$ &$34~(0.74)$ &$33~(3.19)$ \\ 
			&$10$ &$35~(0.06)$ &$36~(0.07)$ &$35~(0.2)$ &$34~(0.85)$ &$33~(3.69)$ \\ 
			\hline 
		\end{tabular} 
		\caption{Number of iterations and wall clock solve time for $\alpha = 1$} 
		\label{table:iop-eg} 
	\end{center} 
\end{table} 

